Autonomous Cooperative Flight Control for Airship Swarms

This work investigates two approaches for the design of autonomous cooperative flight controllers for airship swarms. The first controller is based on formation flight and the second one is based on swarm intelligence strategies. In both cases, the team of airships needs to perform two different tasks: waypoint path following and ground moving target tracking. The UAV platform considered in this work is the NOAMAY airship developed in Brazil. We use a simulated environment to test the proposed approaches. Results show the inherent flexibility of the swarm intelligence approach on both tasks.

==> Guidance.tex <==
\section{Guidance and Control Approaches}
\label{sec:control}

\subsection{Second Layer - Kinematic Based Guidance}
For the middle layer (guidance), we use here the ``leader-follower'' coordinated flight approach. Although extensively investigated for different kinds of aircrafts, to our knowledge, there is only one work in the literature focused on coordinated flight of airships, and using the ``leader-follower'' approach, that is the one presented in the ``\emph{Airship Formation Control}'' \cite{bicho2006airship} paper. However, this work is only applied to the waypoint path following case and, besides, the authors do not show the resulting control actuators signals for better analysis and comparison. The idea of the ``leader-follower'' technique is to impose speed and  orientation references for two airships at a time, which may fly in 3 different modes that are: in column, in line or in ``oblique'' formation (\cref{fig:airshipFormation}). The distance and orientation between the two airships are controlled by keeping the heading and relative speed between both, which is guaranteed by the low level controllers. This structure is then combined to generate more complex formations with an arbitrary number of airships, such as the known ``V'' formation. Nevertheless, in this preliminary work, we consider only three airships flying together in ``V'', though we extend the idea of \cite{bicho2006airship} to cover more complex flight mission cases like hovering and moving target tracking. 

\begin{figure}[!htb]
	\centering
	\def\svgscale{.5}
	\input{images/airshipFormation.pdf_tex}
	\caption{Basic airship configurations in a \emph{leader/follower} formation.}
	\label{fig:airshipFormation}
\end{figure}

Consider that $\psi_i$ is the Euler angle orientation (yaw angle), in the D axis ($\mathfrak{I}$ frame) for the \textit{follower} airship and $\zeta_i$ the angle between the \textit{leader} and \textit{follower} positions in the same axis. It is desired that the \textit{follower} airship maintains a certain distance, $\rho_{i,d}$, from the \textit{leader}, as well as a certain relative angle, $\zeta_{i,d} $. The solution for this kind of problem of position/orientation control is delegated to the low level controller (3rd layer of \cref{fig:architecture}) that is based on a simple kinematic model (\cref{eq:modCarro} and \cref{fig:controlErrors}). This {SFKC} approach is commonly used in mobile robotics for terrestrial vehicles (\cite{siegwart2011introduction}). 
 
\begin{equation}
	\begin{bmatrix}
		\dot{\rho}     \\
		\dot{\zeta}    \\
		\dot{\epsilon}
	\end{bmatrix}
	=
	\begin{bmatrix}
		-\cos{\zeta}              & 0  \\
		\frac{\sin{\zeta}}{\rho}  & -1 \\
		-\frac{\sin{\zeta}}{\rho} & 0 
	\end{bmatrix}
	\begin{bmatrix}
		u_{ref}      \\
		r_{ref}
	\end{bmatrix}
	\label{eq:modCarro}
\end{equation} 

\begin{figure}[!htb]
	\centering
	\def\svgscale{.5}
	\input{images/controlErrors.pdf_tex}
	\caption{Polar coordinate system with the origin set at the NED frame of the leader airship, used in the 2nd layer (SFKC), here with $ \rho_{i,d} = \zeta_{i,d} = 0. $}
	\label{fig:controlErrors}
\end{figure}

It is important to remark that \cref{eq:modCarro} assumed the goal at the origin of the inertial frame, which does not incur any loss of generality. The complete relations utilised in the simulator were:
\begin{equation}\label{eq:rho}
	\rho_i = \sqrt{{\Delta P_E}^2 + {\Delta P_N}^2} - \rho_{i,d}
\end{equation}	
\begin{equation}\label{eq:delta}
	\zeta_i = - \psi_i + \atan \frac{\Delta P_E}{\Delta P_N} - \zeta_{i,d} 
\end{equation}	
\begin{equation}\label{eq:epsilon}
	\epsilon_i = - \psi_i - \zeta_i + \psi_{j}
\end{equation}
which takes into consideration that the goal frame is a mobile one. To derive the state feedback gain, first we linearise \cref{eq:modCarro} assuming small-angle errors such that $\cos(\zeta) \simeq 1$ and $\sin(\zeta) \simeq \zeta$. The feedback control law defined by \cite{siegwart2011introduction} is:
\begin{equation}
	u_{ref} = k_\rho \rho  
\end{equation}
\begin{equation}
	r_{ref} = k_{\zeta} \zeta + k_{\epsilon} \epsilon
\end{equation}
which had the subscripts dropped, in order to ease the notation. These velocities compose the airspeed reference command sent to the airship as control inputs, that is:
\begin{equation}\label{eq:SFKCoutput}
	\vect{u}_{a_{ref}}=[u_{ref} \ 0 \ 0 \ 0 \ 0 \ r_{ref}]\T;
\end{equation}
As the use of airspeed control signals infers no loss in generality, the subscript $ a $ will not be employed to ease the notation.

The substitution of these control laws in the linearised model of \cref{eq:modCarro} leads to the following closed-loop state space model:
\begin{equation}\label{eq:modCinCarro}
	\begin{bmatrix}
		\dot{\rho}     \\
		\dot{\zeta}    \\
		\dot{\epsilon}
	\end{bmatrix}
	=
	\begin{bmatrix}
		- k_\rho & 0                   & 0            \\
		0        & -(k_\zeta - k_\rho) & - k_\epsilon \\
		0        & -k_\rho             & 0
	\end{bmatrix}
	\begin{bmatrix}
		\rho   \\
		\zeta \\
		\epsilon
	\end{bmatrix}
\end{equation}
whose dynamic matrix should have stable eigenvalues by choosing $ k_\rho > 0 $, $ k_\epsilon < 0 $ and $ k_\zeta > k_\rho $.

One addition that was made to the {SFKC} was a feedforward to aid the velocity tracking of the follower airship. The velocity reference is the true airspeed of the leader airship $ V_t  = \norm{\vect{v}_a}_2 = \sqrt{u_a^2 + v_a^2 + w_a^2} $. Being $ y_j(k) = [P_{N_j}(k), \ P_{E_j}(k)]\T $ the position of the leader airship at any instant $ k $, then the equilibrium point sought by the follower airship is given by 
\begin{equation}
\begin{split}
    y_{ref}(k) = 
    \begin{bmatrix}
        P_{N_j}(k) - \rho_{i,d} \cos({\psi_j(k) + \zeta_{i,d}}) \\
        P_{E_j}(k) - \rho_{i,d} \sin({\psi_j(k) + \zeta_{i,d}})
    \end{bmatrix}
\end{split}
\end{equation}
and 
\begin{equation}
	V_{t_{ref}} = \frac{y_{ref}(k) - y_{ref}(k-1)}{T_s}
\end{equation}
where $ T_s $ is the sampling time. This also added a feedforward gain $ k_{ff} $ to the controller. With the defined linear conditions, $ u_{ref} = V_{t_{ref}} $. This makes the closed-loop state space model
\begin{equation}\label{eq:modWaypoint}
\begin{split}
	\begin{bmatrix}
		\dot{\rho}     \\
		\dot{\zeta}    \\
		\dot{\epsilon}
	\end{bmatrix}
	=
	\begin{bmatrix}
		- k_\rho & 0                   & 0            \\
		0        & -(k_\zeta - k_\rho) & - k_\epsilon \\
		0        & -k_\rho             & 0
	\end{bmatrix}
	\begin{bmatrix}
		\rho     \\
		\zeta    \\
		\epsilon
	\end{bmatrix} + \\
	\begin{bmatrix}
		k_{ff} & 0 \\
		0      & 0 \\
		0      & 0
	\end{bmatrix} 
	\begin{bmatrix}
		u_{ref} \\
		r_{ref}
	\end{bmatrix}
\end{split}
\end{equation}

One of the most interesting properties of this {SFKC} is that with a single set of tuning control parameters $k_\zeta$, $ k_\rho $, $k_\epsilon$ and $ k_{ff} $ it is possible to implement, with just some small changes, the different operational modes of waypoint flight, hovering flight and ground tracking flight used to execute the two main missions of waypoint path following and target tracking. For the ``follower'' airship in the ``leader/follower'' guidance approach, the ``goal'' point in \cref{fig:controlErrors} will always be the position of its corresponding ``leader'' airship. And for the main leader airship in the ``V'' coordinated flight, the goal may be the next waypoint (in the waypoint flight), the hovering waypoint (in the hovering flight) and the target current position in North$ \times $East coordinates (in the target tracking). In this last case, the idea is to generate a kind of ``walk-stop-walk'' behaviour to follow the target using both the constant airspeed and the hovering control modes. The airship will follow the target at a constant airspeed and whenever its projected distance to the object reaches the limit of 5 m, it switches to the hovering control. 

\vspace{-0.2cm}
\subsection{Third Layer - Sliding Mode Controller}
For the third layer of this control architecture, \cite{moutinho2007modeling} explores linear and nonlinear options. In her work, it is stated that because of the system being linearised around a desired condition, it would not be possible to have a controller that meets the required specifications for ground-hover and target tracking, for example. Since target tracking, path following and ground-hovering are objectives of this work, a nonlinear controller had to be implemented. The Sliding Mode Control (SMC) implemented by \cite{vieira2017controle}, manages to control the coupled airship system (lateral and longitudinal motions) while achieving great robustness, given that the system was always stabilised even with the saturation of the actuators and an airspeed variation range of \SIrange[per-mode=symbol]{3}{13}{\meter\per\second} being thus chosen as the third layer controller. This section will only explore the adaptations made to the SMC for this work's implementation. The core development can be followed at \cite{vieira2017controle}.

As is probably known by the reader, the SMC controller have its gains calculated around certain equilibrium conditions, which means that it really only has peak performance around this condition, despite guaranteeing global stability. The dynamical conditions of the airship, however, are extremely non linear. There are saturations and dynamics on the actuators; a naturally elevated inertia, due to the airship form factor; high lateral wind drag; added mass due to air displaced; underactuation on the side of the airship and many more complications. That is to say that, despite being able to reject any uncertainty or perturbations, the gains calculated for a certain trim condition can have poor performance on different conditions, sometimes even saturating the controller. For that reason, it was decided to utilise a minimisation function, aiming to select the most appropriate gains at each instant of simulation. The following algorithm explains the minimisation function:
\begin{algorithm}
	\TitleOfAlgo{trimMinimization($\vect{u}_{a_{ref}},\vect{V}_{t_e},\mathrm{SMCgains}$)}
	\begin{algorithmic}[1]
		\STATE $\vect{V}_{t_{ref}} \gets \vect{u}_{a_{ref}} - \vect{V}_{t_e}$ \% Vector $ \vect{V}_{t_e} $ will be subtracted of scalar $ u_{a_u} $
		\STATE $[\sim,I] \gets \min(\abs{\vect{V}_{t_{ref}}})$  \% The absolute value \\ of each element of $ \vect{V}_{t_{ref}} $ is calculated and \\ the index of the smallest is saved
		\STATE $k_{SMC} \gets \mathrm{SMCgains}(I)$ \% The gains of \\ the SMC for that trim condition are \\ selected and saved
		\RETURN $k_{SMC}$
	\end{algorithmic}
\end{algorithm}\\
where $\vect{u}_{a_{ref}}$ is the SFKC guidance controller output to the SMC controller (\cref{eq:SFKCoutput}), $\vect{V}_{t_e}$ is a vector that contains 74 different airspeeds - between [0.3-15] m/s - that are used as trim points, $ \mathrm{SMCgains}$ is another vector that contains 74 sets of gains for the SMC controller, related to each trim point and $\vect{V}_{t_{ref}}$ is the reference airspeed. In other words, at each instant the function will choose the closest trim point to the desired airspeed and will send the corresponding set of gains to the SMC controller.

==> Methodology.tex <==
\section{Methodology}
\label{sec:methodology}

The problem of using a swarm of UAVs to track a trajectory or a moving target becomes increasingly complex if the team has also to obey a given flight formation. This turns into an even more challenging task if we consider the difficulties associated to the control of outdoor airships \cite{moutinho2016airship}, \cite{azinheira2006airship}, \cite{Liesk}, \cite{Vieira2017}. 

In this section we present the methodology of the proposed solutions to this problem including the fundamentals of the two cooperative flight control approaches: one based on swarm intelligence and the other based on classical cooperative formation flight \cite{Dong2015}, \cite{Olsen1999}, \cite{bicho2006airship}. 

\subsection{Swarm Intelligence}
\label{subsec:swarm}

In the 1980’s, Beni, Hackwood, and Wang introduced the concept of \textit{swarm intelligence} [Bonabeau et al., 1999]. Swarm intelligence can be defined as the collective intelligence emerging from a group of simple agents. In the wild, many species are known to display \textit{swarm intelligence} behaviour. These behaviours are generally classified as follows [Bonabeau et al., 1999],[Sardinha, 2016], [Koenig and Dickinson, 2017]:

\begin{itemize}
\item Flocking: a flocking behaviour occurs when animals gather and move together as what could seem to be a single organism (e.g, a flock of starlings or a school of mackerels) 
\item Foraging: a foraging behaviour occurs when animals collaborate to exploit their environment (e.g., ants of a colony share the work of harvesting food all around the nest)
\item Collaborative Manipulation: some animals sometimes gather to carry heavy loads (e.g, ants are also known to have such behaviour)
\item Aggregation: some animals sometimes regroup and stay together (e.g., emperor penguins do so to protect themselves from the cold)
\end{itemize}

Biologically inspired strategies can provide better performance to classical approaches in many applications. For instance, in nature there is no global communication system for flocks of birds, schools of fish or ant colonies, but they nevertheless display a form of collective intelligence [Tan and Zheng, 2013]. In recent years, computer scientists have been developing strategies to try and mimic the behaviour of these kinds of insects and animals. Swarm Robotics can be considered one of these strategies, which takes inspiration from the behaviour of insects, such as bees, ants and termites. The simplistic agents that form the swarm are able to communicate with one another, either explicitly, implicitly or through passive action recognition, and have a stochastic behaviour that can generate some sort of collective intelligence (Trianni, 2008), (Sahin, et al. 2008), \cite{Brambilla}.

The main characteristics of swarm robotics are:

\begin{itemize}
\item Robustness: swarm robots are able to continue working and accomplish their mission despite suffering the failure of some of their individual members. This capability is a result of the decentralised distributed architecture that characterises swarms
\item Flexibility: these kinds of systems can adapt easily to changes in the requirements as well as to perturbations in the environment
\item Scalability: given that swarm robotic systems are based on decentralised distributed systems, it is possible to increase the number of agents without sacrificing performance. The computational complexity does not increase with the number of agents since each of them relies on its own independent controller
\item Emergence: the most important property of these kinds of systems is the emergence of a collective intelligent behaviour from simple interactions between the local agents (swarm members) and the environment. Usually each agent follows a set of simple rules, which results into an intelligent behaviour as a group
\end{itemize}

Swarm robotics approaches have been applied to a range of applications for optimization and resource-allocation tasks, including the traveling-salesman problem, job-shop scheduling, vehicle routing, self-repairing formation control for mobile agents, load balancing, searching, autonomic computing in overlay networks and flight coordination \cite{Brambilla}.

In the course of this work two major swarm intelligent strategies are used to establish coordination between the airships: the Boids Algorithm \cite{reynolds1987flocks} and the Robotic Particle Swarm Optimization (RPSO) \cite{couceiro2011novel}. 

\vspace{+10pt}
\subsubsection{Boids Algorithm}

This algorithm has first been designed by Craig Reynolds in \cite{reynolds1987flocks}, in order to simulate a flock of birds in a more realistic way. It is based on three simple rules:

\begin{enumerate}[label=(\roman*)]
\item Collision Avoidance: the members of the flock are not supposed to collide among
themselves (short range \textit{repulsion})
\item Velocity Matching: the members align their speed and direction on their neigh-
bours’ ones (neighbours \textit{mimicking})
\item Flock Centring: the members have to stay together to form a group (long range
\textit{attraction})
\end{enumerate}

\vspace{+5pt}
The Boids algorithm can be resumed as follows. Let us consider a flock of $N$ Boids, which $i^{th}$ Boid’s state is given by:

\begin{equation}
\vect{x}_i = (\vect{p}_i^T,\vect{v}_i^T)^T 
\end{equation}

where $\vect{p}_i$ is the Boid’s position and $\vect{v}_i$ its velocity with respect to a fixed global frame. The state of a Boid at time step $t$ can be written as:

\begin{equation}
\vect{x}_{i,t} = \vect{x}_{i,t-1} + \vect{v}_{i,t}
\end{equation}

The three rules, \textit{collision avoidance/repulsion}, \textit{velocity matching/mimicking} and  \textit{flock centring/attraction} contribute to update each agent's velocity $\vect{v}_i$ at every time step $t$. The update can be expressed by weighted average as:

\begin{equation}
\vect{v}_{i,t}=\delta(\vect{v}_{i,t-1})+(1-\delta)(k_r.\vect{v}_{i,r}+k_m.\vect{v}_{i,m}+k_a.\vect{v}_{i,a})
\end{equation}

where $\vect{v}_{i,t}$ is the velocity of the $i^{th}$ member of the swarm at time $t$, and $\vect{v}_{i,r}$, $\vect{v}_{i,m}$ and $\vect{v}_{i,a}$ represent respectively the computation of the 3 aforementioned rules, \textit{repulsion, mimicking, attraction}. These contributions are weighted by the values $k_r$, $k_m$ and $k_a$, that enable the designer to tune the behaviour of the flock. 

\vspace{+5pt}
The velocities $\vect{v}_{i,r}$, $\vect{v}_{i,m}$ and $\vect{v}_{i,a}$ are defined as follows.

\vspace{+5pt}
Velocity $\vect{v}_{i,r}$:

\begin{equation}
\vect{v}_{i,r}=\sum_{j\in \mathcal{E}}{\frac{\vect{p}_{i,t-1}-\vect{p}_{j,t-1}}{N'-1}}
\end{equation}

where $\vect{p}_{i,t-1}$ is the position of the $i^{th}$ agent at time $t$, and $\mathcal{E}$ and $N'$ can be defined as:

\begin{equation}
\mathcal{E} = {l \in [1, N]  \subset \mathbb{N} \setminus \lVert \vect{p}_{i,t-1}-\vect{p}_{j,t-1} \rVert \leq d_{lim}}
\end{equation}

\begin{equation}
N' = card \lbrace \mathcal{E} \rbrace
\end{equation}

and $d_lim$ sets the limit below which the agents will avoid each other.

\vspace{+5pt}
Velocity $\vect{v}_{i,m}$: 
\begin{equation}
\vect{v}_{i,m}=\sum_{j=1,j\neq i}^{N}{\frac{\vect{v}_{j,t-1}}{N-1}}
\end{equation}

\vspace{+5pt}
Velocity $\vect{v}_{i,a}$:
\begin{equation}
\vect{v}_{i,a}=-\vect{p}_{i,t-1} + \sum_{j=1,j\neq i}^{N}{\frac{\vect{p}_{j,t-1}}{N-1}}
\end{equation}

As can be seen in \textit{Equation 5}, a limit distance $dlim$ corresponds to the distance from which the separation rule starts having an effect on the Boid. Indeed, this separation rule only have a short range effect. The behaviours described by \textit{Equation 7} and \textit{Equation 8} can be enhanced by adding other limit distances. This idea comes directly from natural flocks, where the members only perceive their local environment and closest neighbours, and do not have information from the whole group of animals. The Boids algorithm  has already been successfully implemented on a real robotics swarm, for example in [Saska et al., 2014].

\vspace{+10pt}
\subsubsection{Robotic Particle Swarm Optimization-RPSO}

The second swarm-based approach to the problem is the Robotic Particle Swarm Optimization (RPSO) proposed by Couceiro in \cite{couceiro2011novel} which is based on the PSO. The original PSO algorithm has been developed by Russel Eberhard and James Kennedy in \textbf{[Eberhart and Kennedy, 1995 ???]}. As every optimisation algorithm, it aims at finding the global optimum of a fitness function (also called cost function). It is based on a group of cooperating potential solutions (the particles) moving in the hyperspace of solutions. In other words, each particle can be considered as an explorer moving on a landscape of solutions, and communicating with its teammates to find the best one. 

The RPSO has the advantage of natively including an obstacle avoidance mechanism. The particles are the robots themselves, and the cost function depends on their distance to the target (in the case of a search mission for example). It can be seen as a swarm control algorithm adapted to solve optimisation problems. The robots are controlled by the model described in Equations \ref{eq:rpsoVel} and \ref{eq:rpsoPos}.

\begin{equation}\label{eq:rpsoVel}
\begin{aligned}
\vect{v}_{t+1}&=\vect{a} \otimes \vect{v}_t \\
&+ \vect{b}_1 \otimes  r_1 \otimes  (\vect{p}_{pb,t} - \vect{x}_t)\\
&+ \vect{b}_2 \otimes  r_2 \otimes  (\vect{p}_{nb,t} - \vect{x}_t)\\
&+ \vect{b}_3 \otimes  r_3 \otimes  (\vect{p}_{obs,t} - \vect{x}_t)
\end{aligned}
\end{equation}
\begin{equation}
\vect{x}_{t+1} = \vect{x}_t + \vect{v}_{t+1}
\label{eq:rpsoPos}
\end{equation}
%{\color{red} \textbf{HUGO PLEASE ADD HERE EQUATIONS 2.11 AND 2.12 FROM AUGUSTE'S THESIS
%}}
%On a generic level DPSO employ multiple swarms to avoid local minima that some other methaheuristic approaches suffer from, despite their inherent randomness. These multiple swarms follow Darwin's natural selection principle, where swarms with a higher fitness are likely to generate another particle, whereas swarms that are unable to increase the overall fitness tend to lose particles until the become extinct.



%The \textit{Robotic Particle Swarm Optimization} builds on this concept by introducing the notion of \textit{social exclusion} $SE$ and \textit{social inclusion} $SI$ in the particle swarm domain, since it would be infeasible to delete or spawn robots in real-applications. In this case, and also considering multiple swarms, a counter is set to the number of times a swarm evolves without finding a better solution. If this counter reaches a certain threshold the worst performing robot in that swarm is added to a socially excluded list. On the other hand, if a swarm is able to improve its solution it is rewarded with the best performing robot from the excluded list.

The RPSO for a swarm of N robots in a dynamic environment is described in Algorithm 1. 

{\color{red} \textbf{HUGO @ PLEASE COULD YOU ADD HERE THE "Algorithm 4 RPSO algorithm for a swarm of N robots in a dynamic environment" FROM AUGUSTE'S THESIS (PAGE 79) ?}}

%\begin{algorithm}
%\caption {RDPSO algorithm}
%\begin{algorithmic}[1]
%\FOR{all swarm $S$ in population} 
%\FOR{all robot $r$ in swarm Sn} 
%\STATE Update robot’s evaluation function
%\STATE Update robot’s personal best
%\STATE Move robot according to Equation \ref{eq:rpsoVel} and Equation \ref{eq:rpsoPos}.
%\ENDFOR 
%\IF {Swarm $S$ gets better}
%\STATE Reward swarm S by including the best performing robot of SE in the swarm else
%\ELSE 
%\STATE Punish swarm $S$ by excluding its worst performing robot into $SE$
%\ENDIF
%\STATE Spawn a new swarm with probability $p$ using robots from $SE$
%\STATE Exclude “failed” swarm in $SE$
%\ENDFOR
%\end{algorithmic}
%\end{algorithm}


This algorithm as been shown to work in problems such as: olfactory search \cite{marques2005finding}, overcome obstacle avoidance problems \cite{couceiro2012introducing}  and working under communication constraints \cite{couceiro2012analysis}. 

\subsection{Formation Flight}
\label{subsec:formation}

The second approach used here is the classical cooperative formation flight \cite{Dong2015}, \cite{Olsen1999}, \cite{bicho2006airship}. This strategy is usually based on the classical hierarchy of communication and coordination \cite{tsourdos2010cooperative} of a cooperative mission planning (Figure 3). The top layer defines the mission task allocation, the middle layer is the guidance block that defines the routes/trajectories/references to be followed by each UAV, and the lower layer corresponds to the local controllers that ensure that the UAVs will execute the commanded trajectories/velocities.

\begin{figure}[!thb]
	\centering
	\includegraphics[width=0.98\linewidth]{mission.png}
	\caption{Typical hierarchy of mission planning in coordinated flight. From \protect\cite{tsourdos2010cooperative}.}
	\label{fig:architecture}
\end{figure}

In this work, we focus our investigation in layers 2 (path planning and guidance) and  3 (low level control), as we suppose that the flyable paths or waypoints are given and no optimization on the route/path is executed. However, regarding the path planning, which is a higher level component of the middle layer, we briefly consider it here, for example to generate a better way to approach and stay at a given distance from the searched object in the target tracking task. 

The coordinated formation approach used here is the leader/follower technique, very common on UAVs coordinated flight \cite{Kumar2}, \cite{Dong2015}, \cite{bicho2006airship}. In this mode, the follower airship should maintain a desired distance and orientation angle from the leader, which allows for a flying formation to be achieved, be it in line, column or diagonal (“V" formation). It is implemented here using a State Feedback Kinematic Control (SFKC) approach for layer 2 (guidance), commonly used in mobile robotics for terrestrial vehicles \cite{siegwart2011introduction}. And for the low level (layer 3) we consider an adaptation of the Nonlinear Sliding Mode Control (SMC) of \cite{Vieira2017}, whose purpose is to track the commanded position/orientation/velocity of the autonomous vehicles. 

% We remark that the idea here is not to make a strict comparison of performance of the two techniques (intelligent swarm and formation flight), but indeed to explore the best features of each one that matches the given assignment. Following this principle, the intelligent swarm is applied here to the area coverage case due to its natural behaviour of multiple mobile entities to converge on a single point of interest, disperse, and regroup again.  The classical control is used for the waypoint/hovering task as it is suited to trajectory tracking with accurate position/velocity control. And finally, both approaches are applied to the task of ground target tracking where some analytical comparison can be made. 

Other basic assumptions and hypothesis for this work are presented in the sequel.
We suppose that each airship is provided with the necessary equipment/sensors and network communications for a precise navigation as well as for the recognition and tracking of the ground target. Regarding he mission architecture type, the intelligent swarm is a decentralized architecture, while the formation flight is a semi-decentralized one, when just the “leader” UAV receives external commands, while the other UAVs are distributed autonomously in relation to their closest “companions” \cite{tsourdos2010cooperative}, \cite{Dasgupta2008}. 

The development, test and validation of the approaches will be restricted to the airship computational simulation environment, a 6-DOF dynamic simulator (Simulink/Matlab), based on a high fidelity dynamic model including wind/turbulence and aerodynamic coefficients from wind tunnel experiments \cite{gomes1998airship}, \cite{Paiva2006}, \cite{moutinho2016airship}. For the intelligent swarm design it was used a simplified version of the simulator considering a pseudo-kinematic model \cite{Artaxo2018}, while for the formation flight control we have used the full nonlinear dynamic model. Also, for simulation purposes, and considering the heavy computational effort of multiple airship models, we consider a configuration of 5 airships in the intelligent swarm and 4 airships in the formation flight. Finally, for the intelligent swarm case, we suppose a collision-avoidance that is natural from this technique and for the formation flight we consider a collision-free motion environment \cite{Kumar2}, where each airship flies at a given altitude.

==> TargetTracking.tex <==
\section{Target Tracking}
\label{sec:targettracking}

\subsection{Results}
The second simulation, shown on \cref{fig:waypointDynamicalTargetTracking}, illustrates the case of moving target tracking and \cref{fig:waypointDynamicalTargetTrackingSpeed} shows the corresponding leader's signals. The performance obtained by the leader here is comparable to the kinematic case. The followers also had a good performance, even though their errors were larger than leader had. In this mission, the leader is told to follow a ground target and it does that by engaging successive hovering modes. This way, whenever the target is within a \SI{10}{\meter} radius, the airship will keep still and try to face the wind. With more than \SI{10}{\meter}, the leader will accelerate, trying to close the distance.
\begin{figure}[!htb]
	\centering
	\includegraphics[width=\linewidth]{sim2}
	\caption{Airships in target tracking mission. The airships are drawn every 20 seconds.}
	\label{fig:waypointDynamicalTargetTracking}
\end{figure}
\begin{figure}[!ht]
	\centering
	\includegraphics[width=0.85\linewidth]{waypointDynamicalTargetTrackingErrors}
	\caption{Error plot of the follower airships in moving target mission (\cref{fig:waypointDynamicalTargetTracking}).}
	\label{fig:waypointDynamicalTargetTrackingErrors}
\end{figure}
\begin{figure}[!ht]
	\centering
	\includegraphics[width=0.99\linewidth]{waypointDynamicalTargetTrackingSpeed}
	\caption{Leader's control signals and sideslip angle ($ \beta $) during target tracking (\cref{fig:waypointDynamicalTargetTracking}).}
	\label{fig:waypointDynamicalTargetTrackingSpeed}
\end{figure}
%\vspace{-0.5cm}
\begin{figure}[!ht]
	\centering
	\includegraphics[width=0.85\linewidth]{waypointDynamicalTargetTrackingDynamics}
	\caption{Leader's error and total velocity signals during target tracking (\cref{fig:waypointDynamicalTargetTracking}).}
	\label{fig:waypointDynamicalTargetTrackingDynamics}
\end{figure}

Unlike the previous mission, the leader also does not have information about the target, that it cannot obtain from its sensors. The leader had an average error of \SI{26.28}{\meter} and a standard deviation of \SI{9.08}{\meter}, while the follower airships had an average of position error of \SI{34.60}{\meter} and a standard deviation of \SI{3.40}{\meter}. The error distribution from the followers is shown on \cref{fig:waypointDynamicalTargetTrackingErrors} and from the leader is shown on \cref{fig:waypointDynamicalTargetTrackingDynamics}.
\\
\subsection{Swarm}
\begin{figure}[!htb]
\centering
\includegraphics[width=\linewidth]{boidsRandomTarget.png}
\caption{Target tracking using Reynolds' flocking}
\end{figure}

\begin{figure}[!htb]
\centering
\includegraphics[width=\linewidth]{rpso1.png}
\caption{Target tracking using RPSO (target's velocity is 7.15 m/s)}
\end{figure}

\begin{figure}[!htb]
\centering
\includegraphics[width=\linewidth]{rpso2.png}
\caption{Target tracking using RPSO (target's velocity is 7.22 m/s)}
\end{figure}
